Knowledge Adaptation for Efficient Semantic Segmentation

Both accuracy and efficiency are of significant importance to the task of semantic segmentation. Existing deep FCNs suffer from heavy computations due to a series of high-resolution feature maps for preserving the detailed knowledge in dense estimation. Although reducing the feature map resolution (i.e., applying a large overall stride) via subsampling operations (e.g., pooling and convolution striding) can instantly increase the efficiency, it dramatically decreases the estimation accuracy. To tackle this dilemma, we propose a knowledge distillation method tailored for semantic segmentation to improve the performance of the compact FCNs with large overall stride. To handle the inconsistency between the features of the student and teacher network, we optimize the feature similarity in a transferred latent domain formulated by utilizing a pre-trained autoencoder. Moreover, an affinity distillation module is proposed to capture the long-range dependency by calculating the non-local interactions across the whole image. To validate the effectiveness of our proposed method, extensive experiments have been conducted on three popular benchmarks: Pascal VOC, Cityscapes and Pascal Context. Built upon a highly competitive baseline, our proposed method can improve the performance of a student network by 2.5\% (mIOU boosts from 70.2 to 72.7 on the cityscapes test set) and can train a better compact model with only 8\% float operations (FLOPS) of a model that achieves comparable performances.

==> mybib.bib.1 <==

USAGE:
\bibliographystyle{mybstfile}
\bibliography{cvml,mybibfile}

@STRING{ACCV  = {Proc. Asian Conf. Comp. Vis.}}
@STRING{CVPR  = {Proc. IEEE Conf. Comp. Vis. Patt. Recogn.}}
@STRING{ECCV  = {Proc. Eur. Conf. Comp. Vis.}}
@STRING{BMVC  = {Proc. British Machine  Vis. Conf.}}
@STRING{ICCV  = {Proc. IEEE Int. Conf. Comp. Vis.}}
@STRING{ICIP  = {Proc. IEEE Int. Conf. Image Process.}}
@STRING{ICPR  = {Proc. Int. Conf. Patt. Recogn.}}

@STRING{ICML  = {Proc. Int. Conf. Mach. Learn.}}
@STRING{ICLR  = {Proc. Int. Conf. Learn. Representations}}
@STRING{UAI   = {Proc. Conf. Uncertainty in Artificial Intelli.}}
@STRING{COLT  = {Proc. Annual Conf. Learn. Theory}}


@STRING{IJCAI   = {Proc. Int. Joint Conf. Artificial Intell.}}
@STRING{AAAI    = {Proc. {AAAI} Conf. Artificial Intell.}}


@STRING{AISTATS = {Proc. Int. Conf. Artificial Intell. \& Stat.}}
@STRING{NIPS    = {Proc. Advances in Neural Inf. Process. Syst.}}
@STRING{NIPSW    = {Proc. Advances in Neural Inf. Process. Syst Workshops.}}
@STRING{KDD     = {Proc. {ACM SIGKDD} Int. Conf. Knowledge discovery \& data mining}}

@STRING{MM      = {Proc. {ACM} Int. Conf. Multimedia}}
@STRING{ACMMM   = {Proc. {ACM} Int. Conf. Multimedia}}



@STRING{JMLR    = {J. Mach. Learn. Res.}}
@STRING{ML      = {Mach. Learn.}}
@STRING{MS      = {Management Sci.}}

@STRING{PR      = {Pattern Recogn.}}

@STRING{TAC         = "{IEEE} Trans. Autom. Control"}
@STRING{TCSVT       = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{TSP         = "{IEEE} Trans. Signal Process."}
@STRING{TSTSP       = "{IEEE} J. Sel. Topics Signal Process."}


@STRING{TIT         = "{IEEE} Trans. Inf. Theory"}
@STRING{TKDE        = "{IEEE} Trans. Knowl. Data Eng."}

@STRING{TNN         = "{IEEE} Trans. Neural Netw."}
@STRING{TNNLS       = "{IEEE} Trans. Neural Netw. \& Learn. Syst."}
@STRING{TIP         = "{IEEE} Trans. Image Process."}
@STRING{TMM         = "{IEEE} Trans. Multimedia"}


@STRING{JRA         = "{IEEE} J. Robot. Autom."}
@STRING{TPAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}

@STRING{TRA         = "{IEEE} Trans. Robot. Autom."}
@STRING{TRO         = "{IEEE} Trans. Robot."}
@STRING{TSMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{TSMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{TSMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{TSMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}

@STRING{IEEE_PROC   = "Proc. {IEEE}"}
@STRING{IEEEPROC    = "Proc. {IEEE}"}


@STRING{IJCV  = "Int. J. Comput. Vision"}
@STRING{CVIU  = {Comp. Vis. Image Understanding}}

@STRING{CoRR  = {arXiv: Comp. Res. Repository}}

--
EOF CVML.bib

@inproceedings{Lin2018interwining,
	title={{Multi-Scale Context Intertwining for Semantic Segmentation}
	},
	author={D. Lin and Y. Ji and D. Linschinski and D. Cohen-Or and H. Huang},
	booktitle=ECCV,
	year=2018,
}

@inproceedings{Zhang2018exfuse,
	title={{ExFuse: Enhancing Feature Fusion for Semantic Segmentation}
	},
	author={Z. Zhang and X. Zhang and C. Peng and D. Cheng and J. Sun},
	booktitle=ECCV,
	year=2018
}
@inproceedings{Chen2018deeplabv3plus,
	title={{Encoder-Decoder with Atrous Separable Convolution for Semantic Image Segmentation}},
	author={L-C. Chen and Y. Zhu and G. Papandreou and F. Schroff and H. Adam},
	booktitle=ECCV,
	year=2018
}
@inproceedings{Sandlermobilenetv22018,
	title={{MobileNetV2: Inverted Residuals and Linear Bottlenecks}},
	author={M. Sandler and A. Howard and M. Zhu and A. Zhmoginov and L-C. Chen},
	booktitle={CVPR},
	year=2018
}
@article{Ayinde2018deep,
	title={{Deep Learning of Constrained Autoencoders for
	Enhanced Understanding of Data}},
	author={B. O. Ainde and J. M. Zurada},
	journal=arXiv:1802.00003,
	year=2018
}
@inproceedings{Wang2018nonlocal,
	title={{Non-local Neural Networks}
	},
	author={X. Wang and R. Girshick and A. Gupta and K. He},
	booktitle={CVPR},
	year=2018
}

@article{Chen2017deeplab,
	author = {L-C. Chen and G. Papandreou and I. Kokkinos and K. Murphy and A.L. Yuille},
	title = {{DeepLab: Semantic Image Segmentation With Deep Convolutional Nets,
		Atrous Convolution, And Fully Connected Crfs}},
	journal=TPAMI,
	year=2017
}

@article{Chen2017deeplabv3,
	author = {L-C. Chen and G. Papandreou and F. Schroff and H. Adam},
	title = {{Rethinking Atrous Convolution for Semantic Image Segmentation}},
	journal={arXiv preprint arXiv:1706.05587},
	year=2017
}
@article{Howard2017mobilenet,
	author = {A.G. Howard and M. Zhu and B. Chen and D. Kalenichenko and W. Wang and T. Weyand and M. Andreetto and H. Adam},
	title = {{MobileNets: Efficient Convolutional Neural Networks for Mobile Vision Applications
	}},
	journal={arXiv preprint arXiv:1704.04861},
	year=2017
}

@inproceedings{Chollet2017xception,
	title={{Deep Learning With Depthwise Separable Convolutions}},
	author={F. Chollet},
	booktitle=CVPR,
	year=2017
}
@inproceedings{Yim2017agift,
	title={{A Gift from Knowledge Distillation: Fast Optimization, Network Minimization and Transfer Learning}
	},
	author={J. Yim and D. Joo and J. Bae and J. Kim},
	booktitle=CVPR,
	year=2017
}
@inproceedings{Lin2017refinenet,
	title={{RefineNet}: Multi-Path Refinement Networks for High-Resolution Semantic Segmentation
	},
	author={G. Lin and A. Milan and C. Shen and I. Reid},
	booktitle=CVPR,
	year=2017
}
@inproceedings{Zhao2017psp,
	title={{Pyramid Scene Parsing Network}
	},
	author={H. Zhao and J. Shi and X. Qi and X. Wang and J. Jia},
	booktitle=CVPR,
	year=2017
}
@article{Wu2017resnet38,
	title={{Wider or Deeper: Revisiting the ResNet Model for Visual Recognition}
	},
	author={Z. Wu and C. Shen and A. van den Hengel},
	journal={arXiv preprint arXiv:1611.10080},
	year=2016
}
@article{Badrinarayanan2017segnet,
	title={{SegNet: A Deep Convolutional Encoder-Decoder Architecture For Image Segmentation}},
	author={V. Badrinarayanan and A. Kendall and R. Cipolla},
	journal=TPAMI,
	year=2017
}
@article{Shuai2017dag,
	title={{Scene Segmentation With Dagrecurrent
	Neural Networks}},
	author={B. Shuai and Z. Zuo and B. Wang and G. Wang},
	journal=TPAMI,
	year=2017
}
@article{Huang2017like,
	author =   {Zehao Huang and Naiyan Wang},
	title =    {{Like What You Like: Knowledge Distill via Neuron Selectivity Transfer}},
	journal =  {arXiv preprint arXiv:1707.01219},
	year =     2017
}
@article{Zhao2017icnet,
	author = {H. Zhao and X. Qi and X. Shen and J. Shi and J. Jia},
	title = {{ICNet for Real-Time Semantic Segmentation on High-Resolution Images}},
	journal={arXiv preprint arXiv:1704.08545},
	year = {2017}
}
@article{Abadi2016tensorflow,
	title={{Tensorflow: Large-Scale Machine Learning On Heterogeneous Distributed
	Systems}},
	author={M. Abadi and A. Agarwal and et~al.},
	journal={arXiv preprint arXiv:1603.04467},
	year=2017
}
@article{Paszke2016enet,
	title={{ENet: A Deep Neural Network Architecture for Real-Time Semantic Segmentation
	}},
	author={A. Paszke and A. Chaurasia and S. Kim and E. Culurciello},
	journal={arXiv preprint arXiv:1606.02147},
	year=2016
}
@article{Treml2016sq,
	title={{Speeding Up Semantic Segmentation For Autonomous Driving
	}},
	author={M. Treml and J. Arjona-Medina and T. Unterthiner and R. Durgesh and F. Friedmann and P. Schuberth and A. Mayr and M. Heusel and M. Hofmarcher and M Widrich et~al},
	booktitle=NIPSW,
	year=2016
}
@inproceedings{Zagoruyko2017atnet,
	author = {Sergey Zagoruyko and Nikos Komodakis},
	title = {{Paying More Attention to Attention: Improving the Performance of
	Convolutional Neural Networks via Attention Transfer}},
	booktitle = ICLR,
	url = {https://arxiv.org/abs/1612.03928},
	year = {2017}}

@inproceedings{Lin2015efficient,
	author = {G. Lin and C. Shen and A. van~den Hengel and I. Reid},
	title  = {{Efficient piecewise training of deep structured models for semantic
	segmentation}},
	booktitle   = CVPR,
	year   = 2016
}
@inproceedings{Zheng2015crfasrnn,
	author = {S. Zheng and S. Jayasumana and  B. Romera-Paredes and V. Vineet and Z. Su and D. Du and C. Huang and P. Torr},
	title  = {{Conditional Random Fields as Recurrent Neural Networks}
	},
	booktitle   = ICCV,
	year   = 2015
}

@inproceedings{Cordts2016Cityscapes,
	author = {M. Cordts and M. Omran and S. Ramos and T. Rehfeld and M. Enzweiler and R. Benenson and U. Franke and S. Roth and B. Schiele},
	title  = {{The Cityscapes Dataset For Semantic Urban Scene Understanding}},
	booktitle   = CVPR,
	year   = 2016
}

@inproceedings{Liu2015semantic,
	author = {Z. Liu and X. Li and P. Luo and C.C. Loy and X. Tang},
	title  = {{Semantic Image Segmentation Via Deep Parsing Network}},
	booktitle   = ICCV,
	year   = 2015
}
@inproceedings{Long2015fully,
	author = {J. Long and E. Shelhamer and T. Darrell},
	title  = {{Fully Convolutional Networks For Semantic Segmentation}},
	booktitle   = CVPR,
	year   = 2015
}


@inproceedings{He2015residual,
	author = {K. He and X. Zhang and S. Ren and J. Sun},
	title  = {{Deep Residual Learning For Image Recognition}},
	booktitle   = CVPR,
	year   = 2016
}
@article{Yu2015multiscale,
	author = {F. Yu and V. Koltun},
	title = {{Multi-Scale Context Aggregation by Dilated Convolutions}
	},
	journal={arXiv preprint arXiv:1511.07122},,
	year=2014
}

@article{Hinton2015distill,
	author = {G. Hinton and O. Vinyals and J. Dean},
	title = {{Distilling the Knowledge in a Neural Network}
	},
	journal={arXiv preprint arXiv:1503.02531},,
	year=2015
}

@article{Romero2015fitnets,
	author = {A. Romero and N. Ballas and S.E. Kahou and A. Chassang and C. Gatta and Y. Bengio},
	title = {{FitNets: Hints for Thin Deep Nets}},
	journal={arXiv preprint arXiv:1412.6550},,
	year=2015
}

@article{Everingham2014pascal,
	author = {M. Everingham and S.M.A. Eslami and L.V. Gool and C.K.I. Williams and J. Winn and A. Zisserman},
	title = {{The Pascal Visual Object Classes Challenge – A Retrospective}},
	journal=IJCV,
	year=2014
}


@InProceedings{Mottaghi2014,
	author       = {R. Mottaghi and X. Chen and X. Liu and N. Cho and S. Lee and S. Fidler and R. Urtasun and A. Yuille},
	title        = {{The Role of Context for Object Detection and Semantic Segmentation in the Wild}},
	booktitle    = CVPR,
	year         = {2014},
}
@article{Simonyan2014vggnet,
	author = {K. Simonyan and A. Zisserman},
	title = {{Very Deep Convolutional Networks for Large-Scale Image Recognition
	}},
	journal={arXiv preprint arXiv:1409.1556},,
	year=2014
}
@InProceedings{Hariharan2011semantic,
	author       = {B. Hariharan and P. Arbelaez and L Bourdev and S. Maji and J. Malik},
	title        = {{Semantic Contours From Inverse Detectors}},
	booktitle    = CVPR,
	year         = {2011},
}

@InProceedings{Jangho2018paraphrasing,
	author       = {J. Kim and S. Park and N. Kwak},
	title        = {{Paraphrasing Complex Network: Network Compression via Factor Transfer}},
	booktitle    = NIPS,
	year         = {2018},
}


